Semantically Conditioned Dialog Response Generation via Hierarchical Disentangled Self-Attention

Semantically controlled neural response generation on limited-domain has achieved great performance. However, moving towards multi-domain large-scale scenarios are shown to be difficult because the possible combinations of semantic inputs grow exponentially with the number of domains. To alleviate such scalability issue, we exploit the structure of dialog acts to build a multi-layer hierarchical graph, where each act is represented as a root-to-leaf route on the graph. Then, we incorporate such graph structure prior as an inductive bias to build a hierarchical disentangled self-attention network, where we disentangle attention heads to model designated nodes on the dialog act graph. By activating different (disentangled) heads at each layer, combinatorially many dialog act semantics can be modeled to control the neural response generation. On the large-scale Multi-Domain-WOZ dataset, our model can yield a significant improvement over the baselines on various automatic and human evaluation metrics.

==> [ACL 2019] Disentangling self-attention heads in dialog generation/table.tex <==
\begin{table*}[thb]
\small
\centering
\begin{tabular}{llcccc|c} 
\toprule
\multirow{2}{*}{Dialog-Act} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{Delexicalized}              & Restored           \\ 
\cmidrule{3-7}
                           &                       & BLEU    & Inform & Request & \multicolumn{1}{c|}{Entity F1} & BLEU  \\ 
\midrule
\multirow{2}{*}{None}                            & LSTM~\cite{DBLP:conf/emnlp/BudzianowskiWTC18}                                 & 18.8           & 71.2 & 60.2& 54.8                           & 15.1                              \\
                                                 & 3-layer Transformer~\cite{vaswani2017attention}                         & 19.1           & 71.1 & 59.9& 55.1                           & 15.2                            \\ 
\midrule
\multirow{3}{*}{Tree Act}                         & SC-LSTM~\cite{DBLP:conf/emnlp/WenGMSVY15}              & 20.5           &74.5 & 62.5 & 57.7                           & 16.6                             \\
                                                 & 3-layer Transformer-out                               & 19.9           &74.4 & 61.1 & 57.4                           & 16.0                              \\
                                                 & 3-layer Transformer-in                                & 20.2           &73.8 & 62.1 & 57.3                           & 16.2                            \\ 
\midrule
\multirow{5}{*}{\begin{tabular}[x]{@{}l@{}}Graph Act\\(Predicted)\end{tabular}}                   & 3-layer Transformer-out                               &     22.5     & 80.8  & 64.8   &            64.2      &                      19.3   \\
                                                 & 3-layer Transformer-in                                &       22.7    &  80.4 &  65.1&                64.6           &    19.9                          \\
                                                 & Straight DSA (44 heads)  + 2 x SA          & 22.6           &  80.3  &  67.1  & 65.0                            &         20.0                     \\
                                                 & 2-layer HDSA (7/27 heads) + SA   & 23.2   & \textbf{82.9}  &  \textbf{69.1} & 65.1                  & 20.3               \\

                                                 & 3-layer HDSA (10/7/27 heads)   & \textbf{23.6}   & \textbf{82.9}  &  68.9 & \textbf{65.7}                  & \textbf{20.6}               \\
\midrule
 \multirow{3}{*}{\begin{tabular}[x]{@{}l@{}}Graph Act\\(Groundtruth)\end{tabular}}                    & 3-layer Transformer-in                          &    29.1   & 85.5 &   72.6 &            83.8   &        25.1           \\
                     & Straight DSA (44 heads)  + 2 x SA                    &  29.6     & 86.4  &  75.6 &           84.1     &            25.5    \\
                     & 3-layer HDSA (10/7/27 heads) & \textbf{30.4}   & \textbf{87.9}   &   \textbf{78.0} &        \textbf{86.2}           &    \textbf{26.2}      \\
\bottomrule
\end{tabular}
\caption{Empirical Results on MultiWOZ Response Generation, we experiment with three forms of dialog act, namely none, one-hot and hierarchical.}
\label{tab:generate}
\end{table*}
